Unsupervised Learning for Identifying Events in Active Target Experiments

This article presents novel applications of unsupervised machine learning methods to the problem of event separation in an active target detector, the Active-Target Time Projection Chamber (AT-TPC). The overarching goal is to group similar events in the early stages of the data analysis, thereby improving efficiency by limiting the computationally expensive processing of unnecessary events. The application of unsupervised clustering algorithms to the analysis of two-dimensional projections of particle tracks from a resonant proton scattering experiment on $^{46}$Ar is introduced. We explore the performance of autoencoder neural networks and a pre-trained VGG16 convolutional neural network. We study clustering performance on both data from a simulated $^{46}$Ar experiment, and real events from the AT-TPC detector. We find that a $k$-means algorithm applied to simulated data in the VGG16 latent space forms almost perfect clusters. Additionally, the VGG16+$k$-means approach finds high purity clusters of proton events for real experimental data. We also explore the application of clustering the latent space of autoencoder neural networks for event separation. While these networks show strong performance, they suffer from high variability in their results.

==> custom_work/kmeans_vgg.tex <==
\begin{tabular}{lll}
\toprule
{} & Accuracy &   ARI \\
\midrule
Simulated &     0.70 &  0.89 \\
Filtered  &     0.75 &  0.39 \\
Raw       &     0.59 &  0.17 \\
\bottomrule
\end{tabular}


==> files_from_roberts_thesis/discussion/clustering/clustering.tex <==
\section{Clustering of AT-TPC events}

From the semi-supervised results, we know that we can construct class separating latent spaces. The next challenge is then to expand that insight into the unsupervised clustering of events. Clustering is an intrinsically harder task, owing to the unsupervised nature of the problem. This leads to differing requirements on the representation of the data, as a linearly separable latent space is not necessarily suitable for clustering. 

The most naive approach to clustering our data is to apply a simple clustering algorithm on the latent representation of an algorithm which we know separates our data. Using a pre-trained model is advantageous because they are generally well studied, but may offer less flexibility.  A more sophisticated approach is to use algorithms designed for clustering. These will invariably carry their own assumptions and pitfalls that we have to be wary of. 

In this thesis, we have applied a K-means algorithm to the latent space of a pre-trained VGG16 model as our naive approach. Which means that the K-means assumptions bound this approach. These include that the clusters are distributed as Gaussians in the high-dimensional latent space and that we have a good idea of the number of clusters. We also investigate the more sophisticated mixture of autoencoder (MIXAE) and deep convolutional embedded clustering (DCEC) models, the latter of which fails to cluster AT-TPC data to any degree. However, the MIXAE model achieves promising results, but assumes uniformly distributed classes and requires a good idea of the number of clusters present in the data.

The assumption that we have a good idea of the number of clusters present is problematic for AT-TPC data. In the filtered and full datasets, the amorphous "other" class probably consist of a variety of event types. These were empirically placed in the same class for classification purposes when labelling the data, precisely because the researchers were unable to identify these events.

In this section, we will explore and discuss the clustering of AT-TPC data using a pre-trained network and the MIXAE model. We begin by considering the results from clustering on the pre-trained VGG16 model latent space. 

\subsection{Clustering with a pre-trained network}

What is immediately clear from the results in table \ref{tab:clstr_vgg} is that the VGG16 latent space is able to capture difference between event classes, achieving an adjusted rand index (ARI) score of $>0.88$ on the simulated data against the ground-truth labels. Recall that the ARI is a measure of clustering similarities, adjusted for chance. A particularly interesting aspect of the results in table \ref{tab:clstr_vgg} is the ability to cluster despite the very high-dimensional latent space. As previously mentioned, Euclidean vector distances can be uninformative in high dimensional spaces, as shown by \cite{Aggarwal}. We can explain a part of this behaviour by the fact that a majority, on the order of $\sim 80\%$, of the entries in the latent vectors are zero-valued. However, that leaves some $\sim \num{1.5e3}$ non-zero elements per sample. This space is still very much a high dimensional representation. For the Euclidean distances to have discriminatory power, we must then infer that the space contains some very dense regions in-between regions of minimal density. In such a configuration, the ratios between distances will not tend to unity, and we find some success with K-means clustering. The results for the filtered and full data show worse performance than for the simulated data. However, these results are still promising for the application of clustering algorithms to pre-trained network latent spaces.

To further characterize the performance, we then consider the confusion matrices shown in figure \ref{fig:clster_confmat}. From these matrices, we can infer some interesting properties about the types of events placed in different clusters. It seems that the clustering of the filtered data identifies proton events that occur closer to the detector plane, and so have less developed spirals. We confirm this by visually inspecting the events in those clusters, as illustrated in figure \ref{fig:filtered_vgg_clster_repr}. Similarly, we infer that clustering of full events segments the proton class by the noisiness of the event, placing the more noisy proton events with the amorphous "other" category. We confirm this argument by inspecting the events contained in each cluster, illustrated in figure \ref{fig:full_vgg_clster_repr}.

One of the major strengths of this application is the consistency of the clustering algorithms. The K-means algorithm showed very little, if any, variation in performance when re-running the algorithm. 

\subsection{Clustering with autoencoder based models}

In addition to the results from the VGG16+K-means algorithm, we implemented and applied the DCEC and MIXAE algorithms to the ${}^{46}$Ar data. The former failed to produce any salient clusterings of AT-TPC data. We are confident in the implementation of the algorithm as we are able to reproduce the original author's results on the MNIST handwritten digits dataset. Some value was gained from the experiments, as the mode of failure was informative for the choice to implement the MIXAE algorithm. The DCEC would consistently collapse all samples to one cluster. This exact mode of failure is addressed by the batch entropy loss term introduced in the MIXAE algorithm. Recall from equation \ref{eq:mixae_batch} that the batch entropy encourages the clustering probabilities to be diverse. This also explains the relative imbalance between the weighing of the losses that we found in section \ref{sec:convae_clustering}.

We then turn to the MIXAE performance shown in figures \ref{fig:mixae_sim}, \ref{fig:mixae_clean} and \ref{fig:mixae_full}. From these figures, we observe that while the MIXAE algorithm is able to achieve better performance than the VGG16+K-means algorithm, it suffers from severe stability problems. The results for the simulated data are noteworthy in this regard. To better understand the out of sample performance for the clustering algorithm, we segregate the training and test data entirely for the simulated data. Coupled with the high variability in the simulated performance, we infer that this method may not generalize well to unseen data. Being unsupervised, this is not as big a caveat for the MIXAE as it would be for a supervised algorithm.

Additionally, the best performing algorithms are systematically not those with the lowest loss-values. Indeed it seems that convergence to a perfect one-hot prediction of cluster belonging is indicative of the training having failed. This is especially clear for the filtered and full datasets whose performance are shown in figures \ref{fig:mixae_clean} and \ref{fig:mixae_full} respectively. A defining feature of the loss-plots is in the sample loss, as defined in equation \ref{eq:mixae_sample}. We observe that for the filtered and full datasets, the sample entropy is quite large for the models with the highest performance, with values $S_{sample} > 10$. Together with the observation that the batch-entropy is at a minimum, we conclude that the cluster assignments are near uniform. For comparison, a perfect one-hot representation has a sample loss of $\sim 10^{-1}$. The initially most plausible candidate for this behaviour is the class imbalance in the data, recall from table \ref{tab:class_distr} that the amorphous "other" class represents $\sim 60 \%$ of the full and filtered data. Indeed, we observe that the high performing models on the simulated data have an order of magnitude smaller sample loss compared to the models applied to full and filtered data. 

To further characterize the performance, we inspect the properties of the clustering results achieved by the highest performing models on the filtered and full datasets. The confusion matrices listed in figure \ref{fig:mixae_confmat} initially displays some of the same properties we observed for the VGG16+K-means algorithm. To confirm this behavior, we display some select events from the proton class in figures \ref{fig:filtered_mixae_clster_repr} and \ref{fig:full_mixae_clster_repr}. From these plots, we confirm that while the clustering of the full dataset is in agreement with the VGG16+K-means clusters. That is, we observe noisy proton events being placed in the cluster with the "other" class. This is not the case for the filtered dataset. In the filtered data, the different clusters of proton events do not seem to be visually distinguishable.

\subsection{Comparing clustering methods}

Both the pre-trained and autoencoder based clustering methods hold promise. As is the case for classification, the ease of application of the pre-trained methods is a significant boon, but their static nature creates a hard to breach cap on their performance. We also observe an impressive purity in the proton clusters, as shown in figure \ref{fig:clster_confmat}, for both the filtered and full datasets. Notably, this purity is absent from the MIXAE clustering results. The increase in performance from the VGG16+K-means is then a result of a stronger segmentation of the "other" class of events.


We also observe a link between the clustering and classifying autoencoders in their performance on real AT-TPC data. Recall that for the real data, both the MIXAE and VGG16+K-means approaches showed confusion over very noisy proton events. We observe the same behaviour in the classifying latent spaces of the autoencoder and VGG16 models illustrated by their t-SNE projections shown in figures \ref{fig:vgg_tsne}, \ref{fig:ac_tnse} and \ref{fig:vgg_ac_tnse}.  In those figures, the majority of proton events are correctly segmented from the rest of the data. A portion of the proton events does, however, intermingle with the "other" class in a way that is familiar to us from the clustering results.

It remains to be seen if the algorithms explored in this thesis are capable of separating events in future experiments with more similar tracks. A related avenue for future research is then to combine the autoencoder methods discussed here with a duelling decoder objective on Hough transformed events. This representation is promising as it can explicitly encode the geometry in the event.

For on-going experiments with the AT-TPC, our recommendation for clustering is to employ a pre-trained model combined with K-means. Performance validation is, unfortunately, a necessary step. Some positive identifications of events are thus needed to validate the clustering. 

In this thesis, we have demonstrated strong performance with the MIXAE algorithm. However, further inquiry is needed to investigate the stability of the algorithm. Other avenues of potential interest are the coupling of clustering with a duelling decoder objective, as well as other autoencoder based clustering algorithms. Lastly, there is a need for the coupling of unsupervised performance metrics to measures of performance against ground truth labels.  

==> files_from_roberts_thesis/discussion/discussion.tex <==
\chapter{Discussion}
The primary aim of this chapter is to frame our findings by the goals for our analysis, as presented in sections \ref{sec:clf_procedure} and \ref{sec:cster_procedure}. We divide the discussion of our results by task. First, we will consider the classification performance of our two implemented algorithms on the three different datasets: simulated, filtered and full AT-TPC data. Second, we discuss the unsupervised clustering performance on the same datasets. 


==> files_from_roberts_thesis/results/clustering/clustering.tex <==
\chapter{Clustering of AT-TPC events}\label{chap:clustering}

The principal challenge in the AT-TPC experiments that we are trying to solve is the reliance on labelled samples in the analysis as future experiments may not have as visually dissimilar reaction products  as we observe in the ${}^{46}$Ar experiment.  The  ${}^{46}$Ar experiment does, however, provide a useful example where we can then explore unsupervised techniques. In this chapter, we explore the application of clustering techniques to events represented in latent spaces. 

We begin by exploring a naive K-means approach on the latent space of a pre-trained network. Subsequently, we investigate other clustering methods and two autoencoder based clustering algorithms, as outlined in section \ref{sec:deep_clustering}.

This chapter builds on the previous results from semi-supervised classification. We observe that we can construct high-quality latent spaces. These high-quality spaces facilitate an investigation of clustering techniques. 

The approach for clustering of events is different from the semi-supervised approach in two meaningful ways. First, it is a harder task, as we will demonstrate. The clustering task thus necessitates a more exploratory approach to the problem. Second, as a consequence of the challenge, the focus will be a bit different than for the semi-supervised approach. We will still utilize the same architectures and models starting with a search over the parameter space over which we measure the performance using the adjusted rand score (ARS) and accuracy defined in section \ref{sec:unsupervised_perf} and \ref{sec:supervised_perf}, respectively.

As with chapter  \ref{chap:classification} where we explored the semi-supervised results, we begin this chapter by considering the VGG16 pre-trained model as a benchmark.

Lastly, we note that the focus of this work is mainly on discovering possible avenues for further research. This focus requires a broad scan of possible avenues rather than a rigorous analysis of one specific model.

==> files_from_roberts_thesis/results/clustering/convae.tex <==
\section{Deep clustering algorithms}\label{sec:convae_clustering}

In the previous section we demonstrated a potential for clustering of events from an AT-TPC experiment. To build on this result we will in this section explore the application of the mixture of autoencoders (MIXAE) algorithm introduced in section \ref{sec:deep_clustering}. The other algorithm introduced in section \ref{sec:deep_clustering}, deep clustering with convolutional autoencoders (DCEC), consistently collapsed to just one cluster for all datasets.

In the MIXAE algorithm the hyper-parameters to adjust are all the ordinary parameters that we introduced in table \ref{tab:convae_hyperparams}. In addition to those parameters we have the weighting of the loss terms: $\theta$, $\alpha$ and $\gamma$. These weighting parameters are attached to the reconstruction loss, sample entropy and batch-wise entropy respectively. \cite{Zhang} note that these parameters are very important for the model performance and so we focus primarily on these. 

We empirically freeze the convolutional autoencoder hyperparameters to compress the original $128 \times 128$ to a $8 \times 8$ pixel grid using four convolutional layers. The parameters chosen for the autoencoders are listed in full in table \ref{tab:mixe_ae_hyperparams}.


\begin{table}[H]
\renewcommand*{\arraystretch}{0.5}
\centering
\caption{Hyperparameters selected for the autoencoder components of the MIXAE algorithm, see table \ref{tab:convae_hyperparams} for a full description of the parameters.}\label{tab:mixe_ae_hyperparams}
\setlength{\extrarowheight}{15pt}
\hspace*{-0.5in}
\begin{tabular}{ll}
\toprule
Hyperparameter & Value \\
\midrule
\multicolumn{2}{l}{Convolutional parameters: } \\
\midrule
Number of layers & $4$ \\
Kernels & $[3,\,3,\,3,\,3]$\\
Strides & $[2,\,2,\,2,\,2]$ \\
Filters & $[64,\, 32, \,16, \,8,]$ \\ 
\midrule
\multicolumn{2}{l}{Network parameters: } \\
\midrule
Activation & LReLu \\
Latent type & None \\
Latent dimension & 20  \\
$\beta$ & N/A \\
Batchnorm & False \\
\midrule
\multicolumn{2}{l}{Optimizer parameters: } \\
\midrule
$\eta$ & $10^{-3}$ \\
$\beta_1$ & $0.9$ \\
$\beta_2$ & $0.99$ \\
\bottomrule
\end{tabular}
\end{table}

Since there are then only three remaining hyperparameters we choose to perform a coarse grid-search as described in section \ref{sec:hyperparam_search_arch}.

\begin{table}
\centering
\caption{Hyperparameter grid for the MIXAE loss weighting terms. The grid is given as exponents for logarithmic scales.}\label{tab:mixae_loss_weights}
\begin{tabular}{lll}
\toprule
Parameter & Grid & Scale \\
\midrule 
$\theta$ & $[-1,\, 5]$ & Logarithmic \\
$\alpha$ & $[-5,\, -1]$ & Logarithmic \\
$\gamma$ & $[3,\, 5]$ & Logarithmic
\end{tabular}
\end{table}

\subsection{Simulated AT-TPC data}

To train the MIXAE clustering algorithm, we use the large simulated dataset with $M=80000$ points, evenly distributed between proton- and carbon-events. The algorithm is trained on a subset of $60000$ of these samples, and we track performance on the remaining $20000$ events. 

The grids selected for the search are listed in table \ref{tab:mixae_loss_weights}. The search yielded an optimal configuration with 

\begin{align}
\theta = 10^{-1}, \\
\alpha = 10^{-2}, \\
\gamma = 10^5.
\end{align}

Finally, for these parameters we re-ran the algorithm $N=10$ times to investigate the stability of the algorithm. The results are reported in figure \ref{fig:mixae_sim}. We observe that while the algorithm can achieve very strong performance, with an adjusted rand index (ARI) $ > 0.8$, it fluctuates strongly with repeated experiments. The $ARI$ is a clustering performance measure similar to accuracy, but adjusted for chance. We elaborate on the $ARI$ score in section \ref{sec:unsupervised_perf}. As mentioned in section \ref{sec:mixae} the batch-entropy has a second minimum when the cluster confidences are near equal. It is this behavior we observe in figure \ref{fig:mixae_sim}.

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{./plots/sim_mixae.pdf}
\caption[Clustering performance of MIXAE on simulated AT-TPC data]{Performance for the MIXAE model on simulated AT-TPC data. In the top row the loss components are plotted for each run, and in the bottom row the adjusted rand index (ARI) and clustering accuracy are shown. Each run is color-coded with the ARI achieved at the end of the run. }\label{fig:mixae_sim}
\end{figure}

\subsection{Filtered AT-TPC data}

We repeat the optimization steps in the previous section for the filtered AT-TPC data. The exception being that we allow the algorithm to train on the labelled samples. Beginning with a wide grid equal to the grid used for the simulated data we searched over all parameter configurations to find promising values. We then performed a local search around these values to pin-point the hyperparameter configuration. This search yielded the optimal hyper-parameters 

\begin{align}
\theta &= 10^{1}, \\
\alpha &= 10^{-1}, \\
\gamma &= 3.162\times 10^3.
\end{align}

\noindent The results of the runs are included in figure \ref{fig:mixae_clean}. We observe ghat the highest performing models reach an $ARI > 0.5$, which is higher than the performance achieved by the K-means algorithm applied to the VGG16 latent space. 

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{./plots/clean_mixae.pdf}
\caption[Clustering performance of MIXAE on filtered event AT-TPC data]{Performance for the MIXAE model on filtered AT-TPC data. In the top row the loss components are plotted for each run, and in the bottom row the adjusted rand index (ARI) and clustering accuracy are shown. Each run is color-coded with the ARI achieved at the end of the run.}\label{fig:mixae_clean}
\end{figure}


\subsection{Full AT-TPC data}

As in the two previous sections, we repeat the same procedure of iterative grid searches on the MIXAE loss-weights. Each configuration is re-run a total of $N=10$ times to capture fluctuations in the performance before a final selection is made on the hyperparameters. For the full dataset the MIXAE hyperparameters converge to the same values as for the clean data, i.e. 


\begin{align}
\theta &= 10^{1}, \\
\alpha &= 10^{-1}, \\
\gamma &= 3.162\times 10^3.
\end{align}

\noindent As with the previous datasets we include a plot of the loss curves and performance measures for $N=10$ runs with the same loss-weight parameters, shown in figure \ref{fig:mixae_full}.

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{./plots/real_mixae.pdf}
\caption[Clustering performance of MIXAE on full event AT-TPC data]{Performance for the MIXAE model on un-filtered AT-TPC data. In the top row the loss components are plotted for each run, and in the bottom row the adjusted rand index (ARI) and clustering accuracy are shown. Each run is color-coded with the ARI achieved at the end of the run.}\label{fig:mixae_full}
\end{figure}

\subsection{Comparing performance}

It is also interesting to compare and contrast the clustering results from the MIXAE model with those of the VGG16$+$K-means outside the fairly abstract accuracies and rand scores. It is especially interesting to compare the cluster assignments, as they can inform further research efforts in the clustering of AT-TPC events. We illustrate the clustering with confusion matrices that are shown in figure \ref{fig:mixae_confmat}. From these matrices, we observe that the MIXAE applied to the clean data correctly clusters the noise events. Additionally, it identifies two proton clusters. We observe that these proton clusters are both less pure than the VGG16+K-means clusters and that there does not seem to be a visually meaningful difference between these clusters. The latter is inferred from figure \ref{fig:filtered_mixae_clster_repr}. 

Applied to the real data the MIXAE correctly separates the proton class, however it is unable to separate the carbon events from the amorphous noise events or from the proton cluster. 

\begin{figure}[H]
\centering

	\subfloat{
	\includegraphics[width=0.5\textwidth]{plots/filtered_mixae_conf_mat.pdf}
}
	\hspace{-1cm}
	\subfloat{
	\includegraphics[width=0.5\textwidth]{plots/full_mixae_conf_mat.pdf}
}
\caption[MIXAE - confusion matrices]{Confusion matrices for the MIXAE clustering algorithm on filtered and full AT-TPC events. The true labels indicate samples belonging to the p (proton), carbon (C), or other classes. }\label{fig:mixae_confmat}
\end{figure}

Lastly we wish to further investigate if there are systematic differences between proton events that were placed in different clusters for the clean and full data. From figure \ref{fig:mixae_confmat} we see that the MIXAE algorithm creates two proton clusters for the filtered data, and places about fifty per-cent of the proton events in a cluster with the amorphous "other" events. We extract some proton events from these clusters to inspect whether systematic differences occur. 


\begin{figure}
\centering
\includegraphics[width=\textwidth]{plots/clean_cluster_repr.pdf}
\caption[Selection of carbon events in differing clusters]{Selection of carbon events belonging to different clusters. Each row represents one of the clusters for the filtered data as shown in figure \ref{fig:mixae_confmat}. There seems to be no clear distinction between these rows.}\label{fig:filtered_mixae_clster_repr}	
\end{figure} 

\begin{figure}
\centering
\includegraphics[width=\textwidth]{plots/real_cluster_repr.pdf}	
\caption[Selection of proton events in differing clusters]{Selection of proton events belonging to different clusters. Each row represents one of the clusters for the full data as shown in figure \ref{fig:mixae_confmat}. We observe a tendency for the more noisy events to be placed in the "other" cluster}\label{fig:full_mixae_clster_repr}	
\end{figure} 

==> files_from_roberts_thesis/results/clustering/vgg.tex <==
% !TEX spellckeck=en_GB

\section{Clustering using a pre-trained model}\label{sec:vgg_cluster}

As in chapter \ref{ch:architectures}, we also use the VGG16 pre-trained network as a baseline for the clustering performance. We begin by considering a classical K-means approach to clustering. However, the output from the VGG16 network is very high dimensional with output vectors in $\R^{8192}$. One of the primary concerns is then the curse of dimensionality, where the ratio of distances goes to one with increasing dimensionality as shown by \citet{Aggarwal}. However, one of the central caveats to the authors  finding is that the elements are uniformly distributed in the latent space. It is then possible that all the class information lies in some sub-space of the latent data. To investigate this, we perform clustering analysis using the full representation and the $10^2$ first principal components only. 

\subsection{K-means}

We begin by investigating the K-means clustering algorithm on the VGG16 latent space. As in chapter \ref{chap:classification} the VGG16 model is pre-trained on the imagenet dataset creating a set of vectors $\boldsymbol{x} \in \R^{8192}$. To cluster we use \lstinline{scikit-learn} implementation of the K-means algorithm, with default parameters \cite{Pedregosa2011}. The results of the clustering runs are included in table \ref{tab:clstr_vgg}. We observe that we are able to attain near-perfect clustering on simulated data and that there is a sharp decline in performance as we add noise by moving to the filtered and full datasets. 

\begin{table}[H]
\centering 
\caption[K-means on pre-trained model]{K-means clustering results on AT-TPC event data. We observe that the performance predictably decreases with the amount of noise in the data.}\label{tab:clstr_vgg}
\input{./plots/kmeans_vgg.tex}
\end{table}

In addition to the performance measures reported in table \ref{tab:clstr_vgg}, it is interesting to observe which samples are being wrongly assigned. We achieve this by tabulating the assignments of samples relative to their ground truth labels. From these tables, we can infer which classes are more or less entangled with others. We tabulate the results for each dataset is in figure \ref{fig:clster_confmat}. We observe that the proton class is consistently assigned in a pure cluster. Purity is inferred by how much spread there is in the column between the ground truth labels. A high-quality cluster will, in addition to being pure, also capture most entries the class represented by the cluster. For example, consider the row corresponding to the proton class in figure \ref{fig:clster_confmat}. The column corresponding to the largest entry in the proton row has zero other predicted classes in it. From this, we conclude that the proton cluster is a high quality, high purity cluster. 

\begin{figure}
\centering

	\subfloat{
	\includegraphics[width=0.35\textwidth]{./plots/Simulatedvgg_pca_conf_mat.pdf}

}
	\hspace{-1cm}
	\subfloat{
	\includegraphics[width=0.35\textwidth]{plots/Filteredvgg_pca_conf_mat.pdf}
}
	\hspace{-1cm}
	\subfloat{
	\includegraphics[width=0.35\textwidth]{plots/Fullvgg_pca_conf_mat.pdf}
}
\caption[Pre-trained network - confusion matrices]{Confusion matrices for the K-means clustering of simulated, filtered and full AT-TPC events. The true labels indicate samples belonging to the p (proton), carbon (C), or other classes. }\label{fig:clster_confmat}
\end{figure}

We repeat this analysis using a PCA dimensionality reduction on the latent space of the VGG16 model. This is done to estimate to what degree the class separating information is encoded in the entirety of the latent space, or in some select regions. The results from the PCA analysis were virtually identical to the results sans the PCA, and so we omit them for brevity. 

Furthermore, we wish to characterize further the clusters presented in figure \ref{fig:clster_confmat}. To achieve this, we sample from the proton samples belonging to different clusters for the filtered and full data.

\begin{figure}
\includegraphics[width=\textwidth]{plots/filtered_vgg_cluster_repr.pdf}
\caption[Filtered proton samples by cluster belonging]{Illustrating a sample of proton events from different K-means clusters from the filtered dataset. Each row belongs to a single cluster corresponding to the filtered confusion matrix in figure \ref{fig:clster_confmat}}\label{fig:filtered_vgg_clster_repr}
\end{figure} 

\begin{figure}
\includegraphics[width=\textwidth]{plots/full_vgg_cluster_repr.pdf}
\caption[Full proton samples by cluster belonging]{Illustrating a sample of proton events from different K-means clusters from the full dataset. Each row belongs to a single cluster corresponding to the full confusion matrix in figure \ref{fig:clster_confmat}}\label{fig:full_vgg_clster_repr}
\end{figure} 

In addition to the results presented in this section, we performed clustering with a number of different algorithms included in the \lstinline{scikit-learn} package. None of them provided any notable differences from the K-means results or were significantly worse. Notably, the DBSCAN algorithm failed to provide any useful clustering results. We find this important as one of the significant drawbacks of K-means, and the deep clustering algorithms presented in section \ref{sec:deep_clustering}, is that they are all dependent on pre-determining the number of clusters. This is not the case for DBSCAN. 

==> files_from_roberts_thesis/results/results.tex <==
\chapter{Experimental setup and design}

In this chapter, we describe the semi-supervised classification and clustering results obtained on the three active target time projection chamber (AT-TPC) datasets described in section \ref{sec:data}. The simulated data is used to provide a benchmark for the upper bound on the performance of a given algorithm. This chapter is structured by task first, and algorithm second. As such, we will begin with a consideration of the semi-supervised algorithms before continuing with the clustering task. 

 We explore the models proposed in chapter \ref{ch:autoencoder} on two disparate tasks, one of semi-supervised classification and one of clustering. For each task, we evaluate the performance on each of the datasets using appropriate metrics, which were introduced in section \ref{sec:performance_val}. 

 The primary objective for the ${}^{46}$Ar experiment was to identify resonant proton scattering events, but this thesis explores broader applications than this classification task. This broader picture is explicitly geared to the application of the models discussed in this thesis to other AT-TPC experiments. Following this argument, we measure individual class performance wherever appropriate. 

The machine learning experiments conducted in this thesis was performed using the AI-Hub computational cluster at the University of Oslo.  This resource consists of three machines with four RTX $2080$ Nvidia GPU's (graphics processing unit) each. These cards have $\sim 10$GB of memory available for the allocation of models.

\subsection{Semi-supervised classification procedure}\label{sec:clf_procedure}

Our interest in the semi-supervised classification is three fold. Firstly, it provides a bound on the performance we can expect from the clustering algorithms, as the classifier problem is fundamentally an easier task. In addition to the bounding property, the semi-supervised task proved to be an excellent way to explore the types of algorithms we present in this thesis. Secondly, we wish to characterize the performance as a function of the number of available labelled samples. As previously mentioned, one of the principal challenges with the AT-TPC detector is the cost of finding examples of the positive class, if at all possible. Thirdly, we wish to lay the groundwork for a transfer-learning approach to bridging AT-TPC experiments. Take, for example, resonant proton scattering. This could also be a reaction of interest in a different experiment. Applying models trained to recognize these events in the ${}^{46}$Ar experiment could be a feasible approach. The results from the semi-supervised classification experiments are presented in chapter \ref{chap:classification}

The semi-supervised task is to train an autoencoder model on a large dataset, and evaluate the class separation of the latent space using a logistic regression classifier. We use a logistic regression classifier as we wish to measure qualities of the latent space, and not of the classification per se. To provide an additional benchmark for our algorithms, we measure the performance of a logistic regression classifier using the latent space of a pre-trained image classifier model, which has shown to be effective in the classification of events from the ${}^{46}$Ar experiment \cite{Kuchera2019}.

Intrinsic to the measurement of the semi-supervised performance is the budgeting of how many labelled samples one can feasibly extract. Moreover, the principal limitation of the semi-supervised approach is the assumption that the researchers can identify the event class(es) of interest positively. It is then interesting to quantify the change in model performance as a function of how many labelled samples the classification model has to train on. Bear in mind that the representation that the classification model sees is still trained on the full set of events for a given dataset. 

For reference, the models are described in terms of their hyperparameters in table \ref{tab:convae_hyperparams} for the convolutional autoencoder and table \ref{tab:draw_hyperparams} for the DRAW-analogues. To determine the best hyperparameters, we perform on the order of $\sim 10^2$ runs, each taking on the order of $\sim 10^1$ minutes on a single Nvidia $2080$ GPU. For each configuration of the algorithms, we train a classifier on a subset of the labelled set. Subsequently, this classifier is evaluated on the remainder of the labelled data to estimate the out of sample (OOS) error. The best configuration is then lastly re-trained, and we evaluate the OOS error with k-fold cross validation as outlined in section \ref{sec:performance_val}.

\subsection{Clustering procedure}\label{sec:cster_procedure}

While the semi-supervised classification task provides context and understanding to the AT-TPC experiments, the clustering procedure is a direct attempt at solving challenges associated with these experiments. First and foremost is the challenge of acquiring labelled data of the event of interest. The clustering results are presented in chapter \ref{chap:clustering} 

In contrast to the semi-supervised task, the clustering objective presumes that we have access to no labelled data. However, since the purpose of this thesis is in large part exploratory, we will measure performance on the labelled data provided. We explore the performance of the deep clustering algorithms described in section \ref{sec:deep_clustering} as well as a K-means approach using the latent space of a pre-trained image classifier model. 

The clustering task is intrinsically a more challenging task than that of semi-supervised classification, and so more time was spent exploring algorithms to determine which were suitable for clustering AT-TPC data. Before training each of the algorithms in section \ref{sec:deep_clustering} was first configured to reproduce the results from their respective papers. Subsequently, they were applied to the AT-TPC data, with their autoencoder hyperparameters selected empirically from the semi-supervised task. This was done to enable a focus on the clustering components of the algorithm. In particular, we focus on the weighting parameters of the mixture of autoencoders (MIXAE) clustering algorithm.



==> plots/kmeans_vgg_pca.tex <==
\begin{tabular}{lll}
\toprule
{} & Accuracy &   ARI \\
\midrule
Simulated &     0.97 &  0.89 \\
Filtered  &     0.74 &  0.39 \\
Full      &     0.59 &  0.17 \\
\bottomrule
\end{tabular}

